Principled Reinforcement Learning with Human Feedback from Pairwise or $K$-wise Comparisons

We provide a theoretical framework for Reinforcement Learning with Human Feedback (RLHF). Our analysis shows that when the true reward function is linear, the widely used maximum likelihood estimator (MLE) converges under both the Bradley-Terry-Luce (BTL) model and the Plackett-Luce (PL) model. However, we show that when training a policy based on the learned reward model, MLE fails while a pessimistic MLE provides policies with improved performance under certain coverage assumptions. Additionally, we demonstrate that under the PL model, the true MLE and an alternative MLE that splits the $K$-wise comparison into pairwise comparisons both converge. Moreover, the true MLE is asymptotically more efficient. Our results validate the empirical success of existing RLHF algorithms in InstructGPT and provide new insights for algorithm design. Furthermore, our results unify the problem of RLHF and max-entropy Inverse Reinforcement Learning (IRL), and provide the first sample complexity bound for max-entropy IRL.

==> macro2.tex <==

\newcommand*{\eqnameformat}[1]{%
  \textsf{#1}%
}

\makeatletter
\@ifdefinable{\org@maketag@@@}{%
  \let\org@maketag@@@\maketag@@@
  \renewcommand*{\maketag@@@}[1]{%
    \org@maketag@@@{%
      \@ifundefined{eq@name}{#1}{%
        \begin{tabular}[t]{@{}r@{}}%
          #1\tabularnewline
          \eqnameformat{\@nameuse{eq@name}}%
        \end{tabular}%
      }%
    }%
  }%
}
\newif\ifeqname@star
\newcommand*{\eqname}{%
  \@ifstar{\eqname@startrue\eqname@}{\eqname@starfalse\eqname@}%
}
\newcommand*{\eqname@}[2][]{%
  \gdef\eq@name{#1}%
  \ifx\eq@name\@empty
  \else
    \begingroup
      \@ifundefined{GetTitleString}{%
        \gdef\@currenteqlabelname{#2}%
      }{%
        \GetTitleString{#2}%
        \global\let\@currenteqlabelname\GetTitleStringResult
      }%
      \let\@currentlabelname\@currenteqlabelname
      \label{#1}%
    \endgroup
  \fi
  %
  \gdef\eq@name{#2}%
  \ifx\eq@name\@empty
    \global\let\eq@name\relax
  \else
    \ifeqname@star
      \gdef\eq@name{\llap{#2}}%
    \fi
  \fi
}
\@ifdefinable{\org@make@display@tag}{%
  \let\org@make@display@tag\make@display@tag
  \def\make@display@tag{%
    \@ifundefined{@currenteqlabelname}{}{%
      \let\@currentlabelname\@currenteqlabelname
    }%
    \org@make@display@tag
  }%
}
\let\eq@name\relax
\let\@currenteqlabelname\relax
\g@addto@macro\displ@y@{%
  \global\let\eq@name\relax
  \global\let\@currenteqlabelname\relax
}
\@ifdefinable{\org@math@cr@@}{%
  \let\org@math@cr@@\math@cr@@
  \def\math@cr@@[#1]{%
    \org@math@cr@@[{#1}]%
    \noalign{%
      \global\let\eq@name\relax
    }%
  }%
}
\@ifdefinable{\org@eqref}{%
  \let\org@eqref\eqref
  \renewcommand*{\eqref}[1]{%
    \begingroup
      \let\eq@name\relax
      \org@eqref{#1}%
    \endgroup
  }%
}
\g@addto@macro\equation{%
  \eqname{}%
}
\makeatother

\interfootnotelinepenalty=10000  %To ensure that no footnote overflows on to the next page

\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\bean}{\begin{eqnarray*}}
\newcommand{\eean}{\end{eqnarray*}}
\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
\newcommand{\blem}{\begin{lemma}}
\newcommand{\elem}{\end{lemma}}
\newcommand{\bthm}{\begin{thm}}
\newcommand{\ethm}{\end{thm}}

\newcommand{\rhoham}{\ensuremath{\rho_H}}

\newcommand{\red}[1]{\textcolor{red}{#1}}

%\newcommand\Wtilde{\stackrel{\tilde{}}{\smash{M}\rule{0pt}{1.1ex}}}
\newcommand{\fix}{\marginpar{FIX}}
\newcommand{\new}{\marginpar{NEW}}
\newcommand{\sign}{\textrm{sign}}
\newcommand{\cardvsord}{\stackrel[\textrm{cardinal}]{\textrm{ordinal}}{\gtrless}}
\newcommand{\Ind}{\mathbf{1}}
\newcommand{\dist}{\mathcal{F}}
\newcommand{\numitems}{d}
\newcommand{\wt}{w}
\newcommand{\lemmawt}{z}
\newcommand{\unitvec}{e}
\newcommand{\obscard}{Y}
\newcommand{\obsordu}{U}
\newcommand{\obsordv}{V}
\newcommand{\markord}{^{(o)}}
\newcommand{\markcard}{^{(c)}}
\newcommand{\studa}{a}
\newcommand{\studb}{b}
\newcommand{\studc}{c}
\newcommand{\noisestd}{\sigma}
\newcommand{\noisestdo}{\noisestd_o}
\newcommand{\noisestdc}{\noisestd_c}
\newcommand{\eps}{\epsilon}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\obs}{y}
\newcommand{\packdmin}{\alpha}
\newcommand{\diff}{x} %differencing vector
\newcommand{\diffdirect}{u}
\newcommand{\diffmx}{X} %=[\diff_1^T\\ \diff_2^T \\ \vdots \\ \diff_\numobs^T]
\newcommand{\Lnormsqr}[3]{(#1-#2)^T #3 (#1-#2)}
\newcommand{\Lnormd}[3]{\|#1-#2\|_{#3}}
\newcommand{\Lnorm}[2]{\|#1\|_{#2}}
\newcommand{\loss}{\ell}
\newcommand{\epsvec}{\boldsymbol{\epsilon}}
\newcommand{\minimax}{\mathfrak{M}}
\newcommand{\tstone}{{\sc Thurstone}\xspace}
\newcommand{\dir}{{\sc Cardinal}\xspace}
\newcommand{\pair}{{\sc Paired Cardinal}\xspace}
\newcommand{\btl}{{\sc BTL}\xspace}
\newcommand{\ord}{{\sc Ordinal}\xspace}
\newcommand{\mwise}{{\sc $\numchoices$-wise}\xspace}

\newcommand{\norm}[1]{\lVert#1\rVert_2}
\newcommand{\inprod}[2]{\ensuremath{\langle #1 , \, #2 \rangle}}
\newcommand{\trace}[1]{\mathrm{tr}(#1)}
\newcommand{\kl}[2]{\ensuremath{D_{\mathrm{KL}}(#1\|#2)}}
\newcommand{\argmax}{\operatornamewithlimits{arg~max}}
\newcommand{\argmin}{\operatornamewithlimits{arg~min}}

\newcommand{\glmcdf}{F}
\newcommand{\glmpdf}{f}
\newcommand{\wmax}{B}
\newcommand{\cdfparam}{\zeta}
\newcommand{\betacard}{0.13}
\newcommand{\alphacard}{0.15}
% \newcommand{\qed}{\hfill$\blacksquare$}

\newcommand{\maxdiag}[1]{\|{\rm diag}(#1)\|_{\infty}}

\newcommand{\numchoices}{\ensuremath{K}} %number of choices presented to user in general models. For pairwise comparisons, \numchoices=2
\newcommand{\hessgencdf}{\ensuremath{H}} %lower bound on the hessian of the log cdf for general models
\newcommand{\genlapmx}{\ensuremath{L}} %The laplacian matrix for the m-wise comparisons case
\newcommand{\genlapmxinv}{\ensuremath{L^\dagger}}
\newcommand{\rankminusonemx}{M}

% WIDEBAR COMMAND
\newlength{\widebarargwidth}
\newlength{\widebarargheight}
\newlength{\widebarargdepth}
\DeclareRobustCommand{\widebar}[1]{%
  \settowidth{\widebarargwidth}{\ensuremath{#1}}%
  \settoheight{\widebarargheight}{\ensuremath{#1}}%
  \settodepth{\widebarargdepth}{\ensuremath{#1}}%
  \addtolength{\widebarargwidth}{-0.3\widebarargheight}%
  \addtolength{\widebarargwidth}{-0.3\widebarargdepth}%
  \makebox[0pt][l]{\hspace{0.3\widebarargheight}%
    \hspace{0.3\widebarargdepth}%
    \addtolength{\widebarargheight}{0.3ex}%
    \rule[\widebarargheight]{0.95\widebarargwidth}{0.1ex}}%
  {#1}}

%%% New version of \caption puts things in smaller type, single-spaced 
%%% and indents them to set them off more from the text.
\makeatletter
\long\def\@makecaption#1#2{
        \vskip 0.8ex
        \setbox\@tempboxa\hbox{\small {\bf #1:} #2}
        \parindent 1.5em  %% How can we use the global value of this???
        \dimen0=\hsize
        \advance\dimen0 by -3em
        \ifdim \wd\@tempboxa >\dimen0
                \hbox to \hsize{
                        \parindent 0em
                        \hfil 
                        \parbox{\dimen0}{\def\baselinestretch{0.96}\small
                                {\bf #1.} #2
                                %%\unhbox\@tempboxa
                                } 
                        \hfil}
        \else \hbox to \hsize{\hfil \box\@tempboxa \hfil}
        \fi
        }
\makeatother

\newcommand{\widgraph}[2]{\includegraphics[keepaspectratio,width=#1]{#2}}

\newcommand{\order}{\ensuremath{\mathcal{O}}}

\newcommand{\mprob}{\ensuremath{\mathbb{P}}}

\newcommand{\wtvec}{\ensuremath{w}}
\newcommand{\real}{\ensuremath{\mathbb{R}}}

\newcommand{\defn}{\ensuremath{: \, = }}

\newcommand{\Exs}{\ensuremath{\mathbb{E}}}

\newcommand{\wthat}{\ensuremath{\widehat{\scriptsize \wt}}}
\newcommand{\wthatML}{\widehat{\wt}_{\mbox{\scalebox{.6}{ML}}}}
\newcommand{\wtstar}{\ensuremath{\wt^*}}

\newcommand{\ones}{\ensuremath{1}}
\newcommand{\zeros}{\ensuremath{0}}

\newcommand{\gvec}{\ensuremath{g}} 
\newcommand{\kull}[2]{\ensuremath{D_{\mathrm{KL}}(#1\|#2)}}


%% Martin comment
%\newcommand{\mjwcomment}[1]{{{\bf{{\red{{MJW --- #1}}}}}}}
%\newcommand{\mjwcommenta}[1]{{\bf{{\color{lightred}{{MJW --- #1}}}}}}
%
%% Siva comment
%\newcommand{\sbcomment}[1]{{\bf{{\red{{SB --- #1}}}}}}
%\newcommand{\sbcommenta}[1]{{\bf{{\color{lightred}{{SB --- #1}}}}}}
%
%% Nihar comment
%\newcommand{\nscomment}[1]{{\bf{{\red{{NS --- #1}}}}}}
%\newcommand{\nscommenta}[1]{{\bf{{\color{lightred}{{NS --- #1}}}}}}

%%%Remove comments for final version
% Martin comment
\newcommand{\mjwcomment}[1]{}%{{\bf{{\red{{MJW --- #1}}}}}}}
\newcommand{\mjwcommenta}[1]{}%{\bf{{\color{lightred}{{MJW --- #1}}}}}}

% Siva comment
\newcommand{\sbcomment}[1]{}%{\bf{{\red{{SB --- #1}}}}}}
\newcommand{\sbcommenta}[1]{}%{\bf{{\color{lightred}{{SB --- #1}}}}}}

% Nihar comment
\newcommand{\nscomment}[1]{}%{\bf{{\red{{NS --- #1}}}}}}
\newcommand{\nscommenta}[1]{}%{\bf{{\color{lightred}{{NS --- #1}}}}}}

\newcommand{\packvec}[1]{\ensuremath{{\wt^{#1}}}}

\newcommand{\LamTil}{\ensuremath{\Lambda^{\dagger}}}
\newcommand{\xtil}{\ensuremath{\widetilde{x}}}

\newcommand{\Pclass}{\ensuremath{\mathcal{P}}}
\newcommand{\genpar}{\ensuremath{\wt}}
\newcommand{\packnum}{\ensuremath{M}}
\newcommand{\SEMINORM}{\ensuremath{\rho}}
\newcommand{\MiniMax}{\ensuremath{\mathfrak{M}}}
\newcommand{\LAPNORM}[1]{\ensuremath{\|#1\|_{\Sigma_{\mathcal{D}}}}}
\newcommand{\LAPNORMINV}[1]{\ensuremath{\|#1\|_{\LapInv}}}
\newcommand{\LambdaInv}{\ensuremath{\Lambda^{\dagger}}}
\newcommand{\vect}{v}

\newcommand{\Wspacebar}{\ensuremath{\bar{\Wspace}}}
\newcommand{\Wspace}{\ensuremath{\mathcal{W}}}

\newcommand{\Wclass}{\Wspace}
\newcommand{\WclassBar}{\Wspacebar}

\newcommand{\Xmat}{\ensuremath{X}}

\newcommand{\regnoise}{\ensuremath{\varepsilon}}

\newcommand{\strongcon}{\ensuremath{\gamma}}

\newcommand{\Lap}{\ensuremath{L}}
\newcommand{\LapInv}{\ensuremath{\Lap^{\dagger}}}

\newcommand{\vtil}{\ensuremath{\widetilde{v}}}
\newcommand{\util}{\ensuremath{\widetilde{u}}}

\newcommand{\nullspace}{\ensuremath{\operatorname{nullspace}}}

\newcommand{\HACKMINIMAX}[1]{\ensuremath{\MiniMax_\numobs
    \big(\textsc{\small{#1}}; \LAPNORM{\cdot}^2 \big)}}
\newcommand{\genminimax}[2]{\ensuremath{\MiniMax_\numobs
    \big(\textsc{\small{#1}}; \Lnorm{\cdot}{#2}^2 \big)}}

\newcommand{\matnorm}[3]{|\!|\!| #1 | \! | \!|_{{#2}, {#3}}}
\newcommand{\matsnorm}[2]{|\!|\!| #1 | \! | \!|_{{#2}}}
\newcommand{\vecnorm}[2]{\| #1\|_{#2}}

\newcommand{\nucnorm}[1]{\ensuremath{\matsnorm{#1}{\footnotesize{\mbox{nuc}}}}}
\newcommand{\fronorm}[1]{\ensuremath{\matsnorm{#1}{\footnotesize{\tiny{\mbox{fro}}}}}}
\newcommand{\opnorm}[1]{\ensuremath{\matsnorm{#1}{\tiny{\mbox{op}}}}}

\newcommand{\plaincon}{\ensuremath{c}}
\newcommand{\cvoconst}{\ensuremath{b}}
\newcommand{\mwiseconst}{\ensuremath{\alpha}}
\newcommand{\wttil}{\ensuremath{\widetilde{\wt}}}

\long\def\comment#1{}

\newcommand{\gendiff}{E}
\newcommand{\diagmx}{D}
\newcommand{\revmx}{R} %reverse matrix
\newcommand{\eigenvalue}[2]{\lambda_{#1}(#2)}
\newcommand{\spanvectors}[1]{{\rm span}(#1)}
\newcommand{\identity}{I}
\newcommand{\diag}[1]{{\rm diag}(#1)}

\newcommand{\graph}{G}
\newcommand{\vertices}{V}
\newcommand{\edges}{E}

\newcommand{\SPECSETgeneral}{\ensuremath{\mathcal{W}}}
\newcommand{\SPECSET}{\ensuremath{{\SPECSETgeneral}_{\wmax}}}
\newcommand{\SPECSETinf}{\ensuremath{{\SPECSETgeneral}_{\infty}}}


\newcommand{\myglmpdf}{\ensuremath{\glmcdf'}}
\newcommand{\mycdftwo}{\ensuremath{\glmcdf''}}

\newcommand{\numitem}{\numitems}

%\newcommand{\LAPNORM}[1]{\ensuremath{\|#1\|_L}}

%\newcommand{\wtstar}{\ensuremath{\wt^*}}

\newcommand{\wtMLE}{\wthatML}

\newcommand{\lemstrongcon}{\ensuremath{\kappa}}

\newcommand{\Vvar}{\ensuremath{V}}
\newcommand{\Vtil}{\ensuremath{\widetilde{\Vvar}}}
